The Effect of External Debt on Greenhouse Gas Emissions

We estimate the causal effect of external debt on greenhouse gas emissions in a panel of 78 emerging market and developing economies over the 1990-2015 period. Unlike previous literature, we use external instruments to address the potential endogeneity in the relationship between external debt and greenhouse gas emissions. Specifically, we use international liquidity shocks as instrumental variables for external debt. We find that dealing with the potential endogeneity problem brings about a positive and statistically significant effect of external debt on greenhouse gas emissions: a 1 percentage point (pp.) rise in external debt causes, on average, a 0.5% increase in greenhouse gas emissions. One possible mechanism of action could be that, as external debt increases, governments are less able to enforce environmental regulations because their main priority is to increase the tax base to pay increasing debt services or because they are captured by the private sector who owns that debt and prevented from tightening such regulations.

==> stats.tex <==
% Table generated by Excel2LaTeX from sheet 'Table with labels'
\begin{tabular}{p{16.28em}cccccccc}
\toprule
\multicolumn{1}{c}{Variable} & \multicolumn{1}{p{5.39em}}{Obs} & \multicolumn{1}{p{5.39em}}{Mean} & \multicolumn{1}{p{5.39em}}{SD} & \multicolumn{1}{p{5.39em}}{Min} & \multicolumn{1}{p{5.39em}}{p25} & \multicolumn{1}{p{5.39em}}{p50} & \multicolumn{1}{p{5.39em}}{p75} & \multicolumn{1}{p{5.39em}}{Max} \\
\midrule
log of per capita CO2 emissions\newline{}(thousand metric tons) & 1314  & -6.97 & 1.33  & -10.59 & -8.00 & -6.86 & -5.90 & -4.43 \\
\midrule
Index of policy and institutions for environmental sustainability & 319   & 3.12  & 0.46  & 2.00  & 3.00  & 3.00  & 3.50  & 4.00 \\
\midrule
External Debt (\% GDP) & 1314  & 52.55 & 39.68 & 1.16  & 25.80 & 42.28 & 66.42 & 305.99 \\
\midrule
log of real GDP per capita at \newline{}chained PPPs (in 2011US\$) & 1314  & 8.39  & 0.92  & 6.06  & 7.73  & 8.43  & 9.17  & 10.27 \\
\midrule
Industry, value added (\% of GDP) & 1314  & 28.52 & 10.26 & 6.09  & 21.98 & 26.55 & 33.05 & 72.15 \\
\midrule
Agriculture, value added (\% of GDP) & 1314  & 16.70 & 11.53 & 1.74  & 7.17  & 14.01 & 23.82 & 63.83 \\
\midrule
Human capital index & 1314  & 2.09  & 0.55  & 1.05  & 1.62  & 2.05  & 2.53  & 3.36 \\
\midrule
Renewable energy consumption \newline{}(\% of total final energy consumption) & 1314  & 45.15 & 30.69 & 0.07  & 14.37 & 44.21 & 75.13 & 98.34 \\
\midrule
Fossil fuel energy consumption \newline{}(\% of total) & 1314  & 53.71 & 31.11 & 0.00  & 24.26 & 55.90 & 84.91 & 99.98 \\
\midrule
log of Energy use \newline{}(kg of oil equivalent per capita) & 1314  & 6.47  & 0.77  & 2.26  & 5.98  & 6.39  & 6.93  & 8.55 \\
\midrule
Forest area (\% of land area) & 1314  & 32.23 & 21.78 & 0.05  & 13.62 & 31.02 & 49.75 & 94.22 \\
\midrule
Domestic credit to private sector \newline{}(\% of GDP) & 1314  & 29.53 & 26.36 & 0.49  & 11.30 & 21.73 & 37.72 & 145.56 \\
\midrule
KOF Financial Globalization Index & 1314  & 48.85 & 13.19 & 11.29 & 39.75 & 49.98 & 57.80 & 86.73 \\
\midrule
KOF Trade Globalization Index & 1314  & 43.84 & 14.61 & 12.73 & 32.48 & 43.04 & 54.72 & 84.52 \\
\midrule
Net capital inflows (\% GDP) & 1233  & -3.62 & 7.08  & -54.13 & -6.46 & -3.31 & -0.50 & 44.00 \\
\midrule
GDP growth (annual \%)) & 1314  & 0.04  & 0.04  & -0.17 & 0.02  & 0.04  & 0.06  & 0.24 \\
\midrule
Alternative and nuclear energy \newline{}(\% total) & 1286  & 4.23  & 6.21  & 0.00  & 0.57  & 2.30  & 5.38  & 55.58 \\
\midrule
Urban Population (\% total) & 1314  & 48.35 & 20.15 & 9.18  & 32.28 & 46.11 & 64.31 & 91.38 \\
\bottomrule
\end{tabular}%


==> table_lnco2_emi_tot.tex <==
                &\multicolumn{1}{c}{FE}&\multicolumn{1}{c}{IV 2nd stage}&\multicolumn{1}{c}{IV 1st stage}\\\cmidrule(lr) {2-2}\cmidrule(lr) {3-3}\cmidrule(lr) {4-4}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
External Debt (\% GDP)&    0.000         &    0.005\sym{***}&                  \\
                &  (0.000)         &  (0.001)         &                  \\
\addlinespace
Dependent variable (-1)&    0.578\sym{***}&    0.569\sym{***}&    0.018         \\
                &  (0.078)         &  (0.071)         &  (4.794)         \\
\addlinespace
GDP per capita  &    0.184         &    0.839\sym{***}& -117.328\sym{***}\\
                &  (0.196)         &  (0.272)         & (26.316)         \\
\addlinespace
GDP per capita $^2$&   -0.013         &   -0.054\sym{***}&    7.093\sym{***}\\
                &  (0.012)         &  (0.017)         &  (1.599)         \\
\addlinespace
Industry, value added (\% GDP)&    0.002\sym{*}  &    0.009\sym{***}&   -1.218\sym{***}\\
                &  (0.001)         &  (0.002)         &  (0.230)         \\
\addlinespace
Agriculture, value added (\% GDP)&   -0.003         &   -0.004\sym{**} &    0.143         \\
                &  (0.002)         &  (0.002)         &  (0.287)         \\
\addlinespace
Human capital index&   -0.071         &   -0.123         &   15.512         \\
                &  (0.104)         &  (0.076)         & (11.807)         \\
\addlinespace
Renewable energy (\% total)&   -0.008\sym{***}&   -0.003         &   -1.234\sym{***}\\
                &  (0.003)         &  (0.002)         &  (0.254)         \\
\addlinespace
Fossil fuel energy (\% total)&    0.007\sym{**} &    0.016\sym{***}&   -1.748\sym{***}\\
                &  (0.003)         &  (0.004)         &  (0.277)         \\
\addlinespace
Energy consumption (kg per capita)&    0.291\sym{***}&    0.381\sym{***}&  -17.697\sym{***}\\
                &  (0.085)         &  (0.068)         &  (6.126)         \\
\addlinespace
Forest area (\% land area)&   -0.004         &    0.000         &   -0.929\sym{**} \\
                &  (0.003)         &  (0.003)         &  (0.473)         \\
\addlinespace
Credit to private sector (\% GDP)&    0.000         &   -0.001\sym{*}  &    0.347\sym{***}\\
                &  (0.001)         &  (0.001)         &  (0.077)         \\
\addlinespace
Financial Globalization Index&    0.001         &   -0.003\sym{***}&    0.650\sym{***}\\
                &  (0.001)         &  (0.001)         &  (0.143)         \\
\addlinespace
Trade Globalization Index&    0.001         &   -0.003\sym{**} &    0.595\sym{***}\\
                &  (0.001)         &  (0.001)         &  (0.149)         \\
\addlinespace
Net capital inflows (\% GDP)&                  &    0.003\sym{**} &   -0.733\sym{***}\\
                &                  &  (0.001)         &  (0.181)         \\
\addlinespace
GDP growth (annual \%)&                  &    0.565\sym{***}&  -10.110         \\
                &                  &  (0.184)         & (24.290)         \\
\addlinespace
US FFR * Chinn-Ito (Neighbors weighted average)&                  &                  &  -37.011\sym{***}\\
                &                  &                  &  (6.766)         \\
\midrule
Observations    &     1314         &     1233         &     1233         \\
Countries       &   78         &   78         &   78         \\
F first stage   &                  &   29.920         &                  \\
Kleibergen-Paap-rk LM statistic&                  &   24.963         &                  \\
p-value         &                  &    0.000         &                  \\
Anderson-Rubin Test statistic&                  &   19.066         &                  \\
p-value         &                  &    0.000         &                  \\


==> table_lnco2_emi_tot_morecontrols.tex <==
                &\multicolumn{1}{c}{FE}&\multicolumn{1}{c}{IV 2nd stage}&\multicolumn{1}{c}{IV 1st stage}\\\cmidrule(lr) {2-2}\cmidrule(lr) {3-3}\cmidrule(lr) {4-4}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
External Debt (\% GDP)&    0.000         &    0.005\sym{***}&                  \\
                &  (0.000)         &  (0.001)         &                  \\
\addlinespace
Dependent variable (-1)&    0.572\sym{***}&    0.571\sym{***}&   -0.680         \\
                &  (0.079)         &  (0.073)         &  (4.896)         \\
\addlinespace
GDP per capita  &    0.217         &    0.825\sym{***}& -118.436\sym{***}\\
                &  (0.186)         &  (0.262)         & (26.660)         \\
\addlinespace
GDP per capita $^2$&   -0.015         &   -0.053\sym{***}&    7.148\sym{***}\\
                &  (0.011)         &  (0.016)         &  (1.620)         \\
\addlinespace
Industry, value added (\% GDP)&    0.002\sym{*}  &    0.008\sym{***}&   -1.173\sym{***}\\
                &  (0.001)         &  (0.002)         &  (0.232)         \\
\addlinespace
Agriculture, value added (\% GDP)&   -0.003         &   -0.005\sym{**} &    0.180         \\
                &  (0.002)         &  (0.002)         &  (0.294)         \\
\addlinespace
Human capital index&   -0.057         &   -0.111         &   15.218         \\
                &  (0.101)         &  (0.072)         & (11.701)         \\
\addlinespace
Renewable energy (\% total)&   -0.008\sym{***}&   -0.003         &   -1.283\sym{***}\\
                &  (0.003)         &  (0.003)         &  (0.264)         \\
\addlinespace
Fossil fuel energy (\% total)&    0.007\sym{**} &    0.015\sym{***}&   -1.736\sym{***}\\
                &  (0.003)         &  (0.003)         &  (0.286)         \\
\addlinespace
Energy consumption (kg per capita)&    0.321\sym{***}&    0.386\sym{***}&  -17.043\sym{**} \\
                &  (0.095)         &  (0.071)         &  (6.702)         \\
\addlinespace
Forest area (\% land area)&   -0.004         &   -0.000         &   -0.878\sym{*}  \\
                &  (0.003)         &  (0.003)         &  (0.475)         \\
\addlinespace
Credit to private sector (\% GDP)&    0.000         &   -0.001         &    0.318\sym{***}\\
                &  (0.001)         &  (0.001)         &  (0.078)         \\
\addlinespace
Financial Globalization Index&    0.001         &   -0.003\sym{**} &    0.660\sym{***}\\
                &  (0.001)         &  (0.001)         &  (0.147)         \\
\addlinespace
Trade Globalization Index&    0.000         &   -0.002\sym{**} &    0.540\sym{***}\\
                &  (0.001)         &  (0.001)         &  (0.150)         \\
\addlinespace
Alternative and nuclear energy (\% total)&    0.004         &   -0.000         &    0.200         \\
                &  (0.005)         &  (0.004)         &  (0.619)         \\
\addlinespace
Urban Population (\% total)&   -0.005         &   -0.004         &    0.102         \\
                &  (0.003)         &  (0.003)         &  (0.326)         \\
\addlinespace
Net capital inflows (\% GDP)&                  &    0.003\sym{**} &   -0.716\sym{***}\\
                &                  &  (0.001)         &  (0.191)         \\
\addlinespace
GDP growth (annual \%)&                  &    0.538\sym{***}&   -7.639         \\
                &                  &  (0.190)         & (25.775)         \\
\addlinespace
US FFR * Chinn-Ito (Neighbors weighted average)&                  &                  &  -38.310\sym{***}\\
                &                  &                  &  (6.983)         \\
\midrule
Observations    &     1286         &     1205         &     1205         \\
Countries       &   71         &   71         &   71         \\
F first stage   &                  &   30.096         &                  \\
Kleibergen-Paap-rk LM statistic&                  &   25.196         &                  \\
p-value         &                  &    0.000         &                  \\
Anderson-Rubin Test statistic&                  &   17.268         &                  \\
p-value         &                  &    0.000         &                  \\


==> table_lnco2_emi_tot_overlapping_subsample.tex <==
                &\multicolumn{1}{c}{FE}&\multicolumn{1}{c}{IV 2nd stage}&\multicolumn{1}{c}{IV 1st stage}\\\cmidrule(lr) {2-2}\cmidrule(lr) {3-3}\cmidrule(lr) {4-4}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
External Debt (\% GDP)&    0.001\sym{**} &    0.006\sym{**} &                  \\
                &  (0.000)         &  (0.003)         &                  \\
\addlinespace
Dependent variable (-1)&    0.369\sym{***}&    0.298\sym{***}&   14.071         \\
                &  (0.061)         &  (0.090)         &  (8.926)         \\
\addlinespace
GDP per capita  &    2.747\sym{**} &    5.946\sym{***}& -692.508\sym{***}\\
                &  (1.262)         &  (2.158)         &(126.178)         \\
\addlinespace
GDP per capita $^2$&   -0.168\sym{**} &   -0.364\sym{***}&   42.267\sym{***}\\
                &  (0.073)         &  (0.132)         &  (7.723)         \\
\addlinespace
Industry, value added (\% GDP)&   -0.000         &    0.002         &   -0.255         \\
                &  (0.003)         &  (0.003)         &  (0.352)         \\
\addlinespace
Agriculture, value added (\% GDP)&   -0.001         &   -0.002         &    0.251         \\
                &  (0.003)         &  (0.003)         &  (0.531)         \\
\addlinespace
Human capital index&    0.048         &    0.055         &   -5.260         \\
                &  (0.224)         &  (0.185)         & (27.795)         \\
\addlinespace
Renewable energy (\% total)&   -0.018\sym{***}&   -0.018\sym{***}&    0.234         \\
                &  (0.005)         &  (0.003)         &  (0.347)         \\
\addlinespace
Fossil fuel energy (\% total)&    0.004         &    0.006\sym{*}  &   -0.184         \\
                &  (0.004)         &  (0.003)         &  (0.426)         \\
\addlinespace
Energy consumption (kg per capita)&    0.410\sym{***}&    0.500\sym{***}&  -20.113         \\
                &  (0.137)         &  (0.121)         & (12.392)         \\
\addlinespace
Forest area (\% land area)&    0.017         &    0.022\sym{*}  &   -0.508         \\
                &  (0.012)         &  (0.011)         &  (1.057)         \\
\addlinespace
Credit to private sector (\% GDP)&   -0.001         &   -0.002         &    0.446\sym{**} \\
                &  (0.002)         &  (0.002)         &  (0.212)         \\
\addlinespace
Financial Globalization Index&   -0.001         &   -0.004\sym{*}  &    0.631\sym{**} \\
                &  (0.002)         &  (0.002)         &  (0.294)         \\
\addlinespace
Trade Globalization Index&    0.001         &   -0.005         &    1.303\sym{***}\\
                &  (0.002)         &  (0.004)         &  (0.393)         \\
\addlinespace
Net capital inflows (\% GDP)&                  &    0.002         &   -0.581\sym{***}\\
                &                  &  (0.002)         &  (0.136)         \\
\addlinespace
GDP growth (annual \%)&                  &    0.427\sym{**} &   -9.909         \\
                &                  &  (0.193)         & (18.860)         \\
\addlinespace
US FFR * Chinn-Ito (Neighbors weighted average)&                  &                  &  -23.010\sym{***}\\
                &                  &                  &  (6.591)         \\
\midrule
Observations    &      284         &      282         &      282         \\
Countries       &   40         &   38         &   38         \\
F first stage   &                  &   12.188         &                  \\
Kleibergen-Paap-rk LM statistic&                  &    9.239         &                  \\
p-value         &                  &    0.002         &                  \\
Anderson-Rubin Test statistic&                  &    4.317         &                  \\
p-value         &                  &    0.038         &                  \\


==> table_policy_enviro.tex <==
                &\multicolumn{1}{c}{FE}&\multicolumn{1}{c}{IV 2nd stage}&\multicolumn{1}{c}{IV 1st stage}\\\cmidrule(lr) {2-2}\cmidrule(lr) {3-3}\cmidrule(lr) {4-4}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
External Debt (\% GDP)&   -0.000         &   -0.005\sym{**} &                  \\
                &  (0.000)         &  (0.002)         &                  \\
\addlinespace
Dependent variable (-1)&    0.677\sym{***}&    0.737\sym{***}&    9.646\sym{***}\\
                &  (0.047)         &  (0.048)         &  (3.163)         \\
\addlinespace
GDP per capita  &    1.527         &   -1.171         & -523.629\sym{***}\\
                &  (0.968)         &  (1.369)         & (99.125)         \\
\addlinespace
GDP per capita $^2$&   -0.076         &    0.086         &   31.627\sym{***}\\
                &  (0.061)         &  (0.084)         &  (6.227)         \\
\addlinespace
Human capital index&   -0.066         &   -0.261         &  -50.649\sym{***}\\
                &  (0.125)         &  (0.205)         & (14.067)         \\
\addlinespace
Credit to private sector (\% GDP)&   -0.001         &    0.001         &    0.384\sym{***}\\
                &  (0.002)         &  (0.002)         &  (0.137)         \\
\addlinespace
Financial Globalization Index&    0.003\sym{*}  &    0.008\sym{**} &    1.161\sym{***}\\
                &  (0.002)         &  (0.003)         &  (0.285)         \\
\addlinespace
Trade Globalization Index&    0.006\sym{*}  &    0.012\sym{**} &    1.699\sym{***}\\
                &  (0.003)         &  (0.005)         &  (0.487)         \\
\addlinespace
Net capital inflows (\% GDP)&                  &   -0.003\sym{**} &    0.112         \\
                &                  &  (0.001)         &  (0.124)         \\
\addlinespace
GDP growth (annual \%)&                  &   -0.581\sym{*}  &  -69.497\sym{**} \\
                &                  &  (0.321)         & (27.503)         \\
\addlinespace
US FFR * Chinn-Ito (Neighbors weighted average)&                  &                  &  -44.577\sym{***}\\
                &                  &                  &  (8.505)         \\
\midrule
Observations    &      628         &      600         &      600         \\
Countries       &   52        &   50         &   50         \\
F first stage   &                  &   27.469         &                  \\
Kleibergen-Paap-rk LM statistic&                  &   14.292         &                  \\
p-value         &                  &    0.000         &                  \\
Anderson-Rubin Test statistic&                  &    5.911         &                  \\
p-value         &                  &    0.015         &                  \\

